ERU-KG: Efficient Reference-aligned Unsupervised Keyphrase Generation

Unsupervised keyphrase prediction has gained growing interest in recent years. However, existing methods typically rely on heuristically defined importance scores, which may lead to inaccurate informativeness estimation. In addition, they lack consideration for time efficiency. To solve these problems, we propose ERU-KG, an unsupervised keyphrase generation (UKG) model that consists of an informativeness and a phraseness module. The former estimates the relevance of keyphrase candidates, while the latter generate those candidates. The informativeness module innovates by learning to model informativeness through references (e.g., queries, citation contexts, and titles) and at the term-level, thereby 1) capturing how the key concepts of documents are perceived in different contexts and 2) estimating informativeness of phrases more efficiently by aggregating term informativeness, removing the need for explicit modeling of the candidates. ERU-KG demonstrates its effectiveness on keyphrase generation benchmarks by outperforming unsupervised baselines and achieving on average 89\% of the performance of a supervised model for top 10 predictions. Additionally, to highlight its practical utility, we evaluate the model on text retrieval tasks and show that keyphrases generated by ERU-KG are effective when employed as query and document expansions. Furthermore, inference speed tests reveal that ERU-KG is the fastest among baselines of similar model sizes. Finally, our proposed model can switch between keyphrase generation and extraction by adjusting hyperparameters, catering to diverse application requirements.

==> latex/sections/_old_2_introduction.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{latex/figures/ReferencesExample.pdf}
    \caption{An example of the different type of references.}
    \label{fig:ReferencesExample}
\end{figure}


Keyphrases are short sequences of words that describe the core concepts of a document. Automatically predicting keyphrases is a crucial problem, as the outputs can be utilized in various downstream tasks, such as document retrieval \cite{zhai1997fast, gutwin1999improving, jones1999phrasier, witten2009build, fagan2017automatic, boudin-etal-2020-keyphrase} and document visualization \cite{chuang2012without}. There are two approaches for keyphrase prediction, namely \textit{keyphrase extraction} (KE) and \textit{keyphrase generation} (KG). The two approaches differ in the output space, where keyphrase generation additionally predicts absent keyphrases. Since human tend to use both present and absent keyphrases to describe documents, \textit{keyphrase generation} has received much attention in recent years. 


In this work, we focus on \textit{unsupervised keyphrase generation} (UKG). In line with previous work, we target a model that receives a document as input and predicts present and absent keyphrases. The desired UKG model must learn to generate keyphrases without labeled data. Being able to build an UKG model in the unsupervised setting is highly desirable, since labeled data is often expensive and difficult to obtain.

In addition, KG models are expected to be used to process large volumes of documents, as evidenced by their potential applications. For example, when utilized for document visualization or retrieval tasks, these models must efficiently handle entire corpora. Furthermore, generated keyphrases are expected to be \textit{conceptual}, i.e., reflecting real-world concepts. Indeed, our analysis of the human labeled keyphrases within the KP20K dataset reveals that 72.3\% of absent keyphrases can be found as present ones of other documents, or as Wikipedia titles. Given these two factors, it is desirable for KG models to be \textit{time efficient} - to manage large scale data processing, and \textit{reliable} - to ensure the generation of meaningful and conceptual keyphrases.



There are two challenges of building such a keyphrase generation model. The first challenge is \textbf{accurate informativeness evaluation}. Without labeled data, it is not straighforward to determine phrases that represent the core concepts of the given text. The second challenge is \textbf{navigating the phrase output space}. Unlike present keyphrases that can be directly identified within the input text, absent keyphrases must be generated from the broader and unconstrained phrase output space. Consequently, this makes absent keyphrase generation potentially slow, as the model must navigate a vast output space; and less reliable due to the unconstrained output space, which allows for the generation of meaningless or non-conceptual keyphrases.


None of the previous work \textit{fully} address the challenges. Regarding the first challenge, we argue that accurate informativeness evaluation of phrases can be achieved if the perception of community regarding the core concepts of documents are considered. However, most of the previous methods do not explicitly model this dimensionality. A few exceptions are \cite{gollapalli2014extracting, boudin-aizawa-2024-unsupervised}, where citation contexts information are utilized for unsupervised keyphrase prediction. However, the use of only citation contexts may not result in comprehensive representation of the documents' core concepts, since it reflects only the view of researchers 

% Previous work in unsupervised keyphrase prediction presents 4 primary definitions of informativeness (see Section \ref{section:related_work})

% (of other articles), which is a subset of the broader community.

Regarding the second challenge, most existing methods generates keyphrases autoregressively, leading to slow inference speed \cite{wu2022fast}. Moreover, they may produce unreliable keyphrases, since autoregressive models are prone to hallucination. An example of this behavior can be found in Table \ref{table:document_case_study}, where CopyRNN \cite{meng-etal-2017-deep} - an autoregressive model, generates ``underwater optical ice'', which does not represent any real concepts\footnote{An exact search on Google (conducted on 28$^{\text{th}}$ January 2025) for the phrase ``underwater optical ice'' does not bring any results}. To our best knowledge, the only existing method that focuses on improving time-efficiency is PromptKP \cite{wu2022fast}, which employs a non-autoregressive decoding method and achieves significantly speed up. However, the non-autoregressive approach taken by PromptKP does not eliminate the problem of generating unreliable keyphrases and can even worsen it, due to lack of dependency modeling 

% \lamdo{Would be stronger if there are examples, can add in section \ref{table:document_case_study} and refer to it here}. 


To address the above challenges, we propose \textbf{ERU-KG} - an \textbf{E}fficient, Reliable, \textbf{R}eference-based, \textbf{U}nsupervised \textbf{K}eyphrase \textbf{G}eneration model. ERU-KG comprises of two components - an \textit{informativeness} and a \textit{phraseness module}, harnessing two key ideas. \textbf{Firstly}, to comprehensively capture community's perception for accurate informativeness evaluation, we propose to learn to evaluate informativeness of phrases (i.e. train the informativeness module) based on \textit{references}, which are the various contexts where a document is mentioned. In particular, references include queries - reflecting the searchable aspects of documents, citation contexts - reflecting how other authors view the given documents, and titles - reflecting the authors' perception of their own work. An example is provided in Figure \ref{fig:ReferencesExample}, the references suggest that the given document addresses topics such as ``sea ice monitoring'' and ``deep learning''.



\textbf{Secondly}, based on the observation that a large percentage of absent keyphrases appear in other documents as present keyphrases, we propose restricting the phrase output space to include 1) present keyphrases of textually-similar documents (i.e. absent keyphrase candidates) and 2) noun phrases found in the given document (i.e. present keyphrase candidates). By restricting the phrase output space, we create an opportunity for improving both the efficiency and reliability of (absent) keyphrase generation. Although this is a simple idea, we are not aware of any previous work that directly exploits it. Previous studies have utilized existing keyphrases in similar documents \cite{ye-etal-2021-heterogeneous, do-etal-2023-unsupervised}, but these keyphrases are employed as additional information, rather than as absent keyphrase candidates, to enhance accuracy rather than efficiency and reliability.


We summarize the contributions of our paper. \textbf{Firstly}, we propose \textbf{ERU-KG} - an UKG model that 1) leverages reference data to accurately evaluate informativeness of phrases; 2) generate keyphrases efficiently and reliably by reusing present keyphrases extracted from similar documents. \textbf{Secondly}, we conduct \textit{groundtruth-based evaluation} and show that ERU-KG outperforms unsupervised baselines and comes very close the CopyRNN \cite{meng-etal-2017-deep}, a supervised model. \textbf{Finally}, to assess the utility of generated keyphrases, we carry out \textit{retrieval-based evaluation}. Our results show that keyphrases generated by ERU-KG enhance text retrieval performance. \lamdo{When write about the results, can consider writing present keyphrase generation (keyphrase extraction) results and absent keyphrase generation results, this will allow readers to understand that our work can also be used to do keyphrase extraction}



\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{latex/figures/Overview.pdf}
    \caption{Overview of the inference process of \textbf{ERU-KG}. Detailed steps of this process are described in Algorithm \ref{algorithm:eru_kg_inference}}
    \label{figure:overview}
\end{figure*}

==> latex/sections/_old__introduction.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{latex/figures/ReferencesExample.pdf}
    \caption{An example of the different type of references.}
    \label{fig:ReferencesExample}
\end{figure}


Keyphrases are short sequences of words that describe the core concepts of a document. Automatically predicting keyphrases is a crucial problem, as the outputs can be utilized in various downstream tasks, such as document summarization \cite{fagan2017automatic}, document retrieval \cite{zhai1997fast, gutwin1999improving, jones1999phrasier, witten2009build, fagan2017automatic, boudin-etal-2020-keyphrase} and document visualization \cite{chuang2012without}. There are two approaches for keyphrase prediction, namely \textit{keyphrase extraction} (KE) and \textit{keyphrase generation} (KG). The two approaches differ in the output space, where keyphrase generation additionally predicts absent keyphrases. Since human tend to use both present and absent keyphrases to describe documents, \textit{keyphrase generation} has received much attention in recent years. In this work, we focus on \textit{keyphrase generation} in the \textit{unsupervised setting}.

% We may not need this passage
% Most existing work in unsupervised keyphrase extraction and generation produce keyphrases by enforcing two criteria, \textit{phraseness} and \textit{informativeness} \cite{tomokiyo-hurst-2003-language, do-etal-2023-unsupervised}. Unsupervised keyphrase extraction (UKE) models \cite{mihalcea-tarau-2004-textrank, wan2008single, gollapalli2014extracting, florescu-caragea-2017-positionrank, bennani-smires-etal-2018-simple, liang-etal-2021-unsupervised, kong-etal-2023-promptrank} mostly enforce the two criteria sequentially by following a two-stage procedure, namely 1) \textit{candidate extraction} (i.e. \textit{phraseness}) and 2) \textit{candidate ranking} (i.e. \textit{informativeness}). On the other hand, unsupervised keyphrase generation (UKG) models either leverage UKE methods to extract silver-labeled keyphrases to train seq2seq models \cite{shen2022unsupervised, kang-shin-2024-improving}, or enforce the two criteria simultaneously at each generation step \cite{do-etal-2023-unsupervised}.

% generate silver labeled keyphrases by enforcing the two criteria, which are then used to train a seq2seq model. Recently, \cite{do-etal-2023-unsupervised} propose an unsupervised keyphrase generation approach by enforcing the two criteria simultaneously.

Existing work in unsupervised keyphrase prediction presents four primary definitions of \textit{informativeness} (see Section \ref{section:related_work}). However, these approaches overlook an important aspect: how documents are referenced and engaged in different contexts. In this paper, we propose that the key concepts of a document are best revealed by how it is interacted, specifically through the queries that retrieve it, the sentences that cite it, and the titles created for it. For example, as illustrated in Figure \ref{fig:ReferencesExample}, the references suggest that the given document addresses topics such as ``sea ice monitoring'' and ``deep learning''. Therefore, it is desirable to leverage references data to learn a keyphrase generation model.

% We argue that neglecting this interactive dimension can result in a skewed identification of a document's true key concepts. 

Keyphrase generation models are expected to be used to process large volumes of documents, as evidenced by their potential applications. When utilized for document visualization or retrieval tasks, these models must efficiently handle entire corpora. In addition, generated keyphrases are expected to be \textit{conceptual}, i.e., reflecting real-world concepts. Indeed, our analysis of the human labeled keyphrases within the KP20K dataset reveals that 72.3\% of absent keyphrases can be found as present ones of other documents, or as Wikipedia titles. Consequently, it is desirable for KG models to be \textit{time efficient} - to manage large scale data processing, and \textit{reliable} - to ensure the generation of meaningful and conceptual keyphrases.

% Another limitation of current keyphrase generation approaches is their \textit{time efficiency}, as it is important for these models to process large volumes of documents. However, most existing keyphrase generation models rely on a sequence-to-sequence approach, leading to low inference speed \cite{wu2022fast}. Consequently, this negatively impacts their scalability and limits their real-world use.


Considering the above discussion, we propose a new problem: \textbf{E}fficient \textbf{R}eliable \textbf{R}eference-based \textbf{U}nsupervised \textbf{K}eyphrase \textbf{G}eneration (\textbf{ER$^2$U-KG}). In line with existing work on keyphrase generation, we target a model that receives a document \(\boldsymbol{x}\) as input and predicts a list of keyphrases $\{\boldsymbol{y}_1, \boldsymbol{y}_2,...\}$.  The model that addresses this problem must further meet two requirements: 1) in the training phase, it should learn to evaluate the informativeness of phrases by analyzing different ways in which the documents are referenced; and 
2) in the inference phase, it should be time-efficient and reliable.

% , specifically through three types of references—\textit{query} (how documents are searched), \textit{citation context} (how they are cited), and \textit{title} (how their authors names them)


% There are two main technical challenges in solving this problem. The first challenge is \textbf{heterogeneous and noisy references}. References can take various forms, including queries, citation contexts, and titles. These different types of refereces differ in length, expression, and structure, requiring distinct approaches to extract the core ideas of the referenced documents. Furthermore, they are often noisy, meaning they may contain irrelevant or ambiguous information. For instance, the references in Figure \ref{fig:ReferencesExample} not only contain the key concepts of the given document, but also contain non-key information such as ``some literatures'' and ``supplementing''. The second challenge is \textbf{efficiency of absent keyphrase generation}. Unlike present keyphrases that can be directly identified within the input text, absent keyphrases must be generated from the broader phrase output space, significantly increasing the complexity of the task.

There are two main technical challenges in solving this problem. The first challenge is \textbf{heterogeneous references}. Learning to evaluate informativeness of phrases from different types of references is difficult as they differ in length, expression, and structure. This makes designing a one-size-fits-all solution unstraightforward since different types of references may require tailored methods to process and learn from. The second challenge is \textbf{navigating the phrase output space}. Unlike present keyphrases that can be directly identified within the input text, absent keyphrases must be generated from the broader and unconstrained phrase output space. Consequently, this makes absent keyphrase generation potentially slow, as the model must navigate a vast output space; and less reliable due to the unconstrained output space, which allows for the generation of meaningless or non-conceptual keyphrases.

% requiring distinct approaches to extract the core ideas of the referenced documents
% , significantly increasing the complexity of the task.

None of the previous work fully addresses both challenges. Regarding the first challenge, some studies have attempted to use citation contexts and titles. Specifically, CiteTextRank (CTR) \cite{gollapalli2014extracting} and SILK \cite{boudin-aizawa-2024-unsupervised} for citation contexts, as well as TPG \cite{kang-shin-2024-improving} for titles. However, SILK and TPG design heuristics for extracting silver-labeled keyphrases, specific to one type of reference. CiteTextRank, on the other hand, evaluates informativeness of candidates using multiple types of references. Unfortunately, CiteTextRank requires references to be available during inference, which does not fit our problem setting.

% (or \textit{contexts} as originally described in their work)

Regarding the second challenge, most existing methods generates keyphrases autoregressively, leading to slow inference speed. To our best knowledge, the only existing method that focuses on improving time-efficiency is PromptKP \cite{wu2022fast}, which employs a non-autoregressive decoding method and achieves significantly speed up. However, the non-autoregressive approach taken by PromptKP does not eliminate the problem of generating unreliable keyphrases and can even worsen it, due to lack of dependency modeling \lamdo{Would be stronger if there are examples, can add in section \ref{table:document_case_study} and refer to it here}. 


% However, \cite{gollapalli2014extracting} requires citation contexts to be available during inference, which does not fit into our problem setting; while \cite{kang-shin-2024-improving ,boudin-aizawa-2024-unsupervised} rely on specific heuristics to extract silver-labeled keyphrases from titles and citation contexts, respectively, which may limit generalization to other types of references. Additionally, as noted earlier, all unsupervised keyphrase generation methods use sequence-to-sequence models that generate keyphrases token by token. While this approach allows for generating absent keyphrases, it is inherently slow due to the sequential nature of the process.



In order to address the challenges, our work harnesses two key ideas. \textbf{Firstly}, we unify different types of past references into a single dataset. In particular, we build triplets from each reference, by finding the corresponding (positive) documents - those that are explicitly mentioned in the reference (e.g., document in figure \ref{fig:ReferencesExample}); and mining the negative documents - those that are not referred to. The resulting dataset is used to train a term-importance predictor, which learns to assign higher weights to terms that differentiate positive documents from negative ones based on the given reference. This process helps identify key terms while filtering out irrelevant ones. The term-importance predictor is then used as a building block to estimate informativeness of phrases. In particular, it estimates phrase informativeness by aggregating the importance scores of individual terms within the phrase. By unifying diverse reference types into a single dataset for training a term-importance predictor, we eliminate the need for type-specific approach design. This solves the first challenge.

% we solve the first part of the first challenge (i.e. heterogeneous references)

\textbf{Secondly}, based on the observation that a large percentage of absent keyphrases appear in other documents as present keyphrases, we propose restricting the phrase output space to include 1) present keyphrases of textually-similar documents (i.e. absent keyphrase candidates) and 2) nounphrases found in the given document (i.e. present keyphrase candidates). By restricting the phrase output space, we create an opportunity for improving both the efficiency and reliability of (absent) keyphrase generation. Although this is a simple idea, we are not aware of any previous work that directly exploits it. Previous studies have utilized existing keyphrases in similar documents \cite{ye-etal-2021-heterogeneous, do-etal-2023-unsupervised}, but these keyphrases are employed as additional information, rather than as absent keyphrase candidates, to enhance accuracy rather than efficiency and reliability.

We summarize the contributions of our paper. \textbf{Firstly}, we propose a new problem called \textbf{E}fficient \textbf{R}eliable \textbf{R}eference-based \textbf{U}nsupervised \textbf{K}eyphrase \textbf{G}eneration (\textbf{ER$^2$U-KG}), which aims not only at learning to identify key concepts of documents from analyzing past references, but also at generating keyphrases in a time-efficient and reliable manner. \textbf{Secondly}, we design a model for tackling the proposed problem. \textbf{Finally}, we conduct extensive experiments to demonstrate the effectiveness of our method. Specifically, we evaluate ER$^2$U-KG's performance by comparing it to other baselines, not only in the keyphrase generation task but also in two downstream tasks: text retrieval and classification. In these downstream tasks, generated keyphrases are used as additional features to investigate their potential to improve performance.


\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{latex/figures/Overview.pdf}
    \caption{Overview of our proposed model \lamdo{Add real data}}
    \label{figure:overview}
\end{figure*}

==> latex/tables/_old__groundtruth_based_evaluation.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|lrrrrrrrrrrrr|}
\hline
\multicolumn{13}{|c|}{{ \textbf{Present keyphrase generation}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{{ }}                     & \multicolumn{2}{c|}{{ SemEval}}                                                        & \multicolumn{2}{c|}{{ Inspec}}                                                         & \multicolumn{2}{c|}{{ NUS}}                                                           & \multicolumn{2}{c|}{{ Krapivin}}                                                       & \multicolumn{2}{c|}{{ KP20K}}                                                          & \multicolumn{2}{c|}{{ Avg}}                                                   \\ \cline{2-13} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{{ }}}   & \multicolumn{1}{c}{{ F@5}} & \multicolumn{1}{c|}{{ F@10}}          & \multicolumn{1}{c}{{ F@5}} & \multicolumn{1}{c|}{{ F@10}}          & \multicolumn{1}{c}{{ F@5}} & \multicolumn{1}{c|}{{ F@10}}         & \multicolumn{1}{c}{{ F@5}} & \multicolumn{1}{c|}{{ F@10}}          & \multicolumn{1}{c}{{ F@5}} & \multicolumn{1}{c|}{{ F@10}}          & \multicolumn{1}{c}{{ F@5}} & \multicolumn{1}{c|}{{ F@10}} \\ \hline
\multicolumn{1}{|l|}{{ TextRank}}             & { 16}                      & \multicolumn{1}{r|}{{ 20.3}}          & { \textbf{29.3}}           & \multicolumn{1}{r|}{{ \textbf{36.2}}} & { 11.6}                    & \multicolumn{1}{r|}{{ 16.6}}         & { 10.1}                    & \multicolumn{1}{r|}{{ 13.6}}          & { 9.1}                     & \multicolumn{1}{r|}{{ 11.6}}          & { 15.22}                   & { 19.66}                     \\
\multicolumn{1}{|l|}{{ MultiPartiteRank}}     & { 22.3}                    & \multicolumn{1}{r|}{{ 22.5}}          & { 26.3}                    & \multicolumn{1}{r|}{{ 30.3}}          & { 23.7}                    & \multicolumn{1}{r|}{{ 22.2}}         & { 17.9}                    & \multicolumn{1}{r|}{{ 15.9}}          & { 18.3}                    & \multicolumn{1}{r|}{{ 15.9}}          & { 21.7}                    & { 21.36}                     \\
\multicolumn{1}{|l|}{{ EmbedRank}}            & { {\ul 24.5}}              & \multicolumn{1}{r|}{{ {\ul 25.6}}}    & { 28.2}                    & \multicolumn{1}{r|}{{ 33.8}}          & { 24.8}                    & \multicolumn{1}{r|}{{ 22.9}}         & { 18.9}                    & \multicolumn{1}{r|}{{ 18.1}}          & { 19.7}                    & \multicolumn{1}{r|}{{ 17}}            & { {\ul 23.22}}             & { {\ul 23.48}}               \\ \hline
\multicolumn{1}{|l|}{{ AutoKeyGen}}           & { 22.1}                    & \multicolumn{1}{r|}{{ 24.3}}          & { 23.2}                    & \multicolumn{1}{r|}{{ 23.7}}          & { 25.7}                    & \multicolumn{1}{r|}{{ \textbf{27}}}  & { 20.6}                    & \multicolumn{1}{r|}{{ {\ul 18.7}}}    & { 20.3}                    & \multicolumn{1}{r|}{{ {\ul 19}}}      & { 22.38}                   & { 22.54}                     \\
\multicolumn{1}{|l|}{{ UOKG}}                 & { 21.9}                    & \multicolumn{1}{r|}{{ 22.3}}          & { 23.4}                    & \multicolumn{1}{r|}{{ 22.8}}          & { {\ul 27.7}}              & \multicolumn{1}{r|}{{ 26.1}}         & { \textbf{21.5}}           & \multicolumn{1}{r|}{{ 17.9}}          & { {\ul 20.9}}              & \multicolumn{1}{r|}{{ 17.6}}          & { 23.08}                   & { 21.34}                     \\
\multicolumn{1}{|l|}{{ \textbf{ERU-KG}}}      & { \textbf{27.3}$^{\dagger \ddagger}$}           & \multicolumn{1}{r|}{{ \textbf{29.4}$^{\dagger \ddagger}$}} & { {\ul 29.2}$^{\dagger \ddagger}$}              & \multicolumn{1}{r|}{{ {\ul 35.3}$^{\dagger \ddagger}$}}    & { \textbf{28.4}}           & \multicolumn{1}{r|}{{ {\ul 26.7}}}   & { {\ul 20.9}}              & \multicolumn{1}{r|}{{ \textbf{19.1}$^{\dagger}$}} & { \textbf{22.2}$^{\dagger \ddagger}$}           & \multicolumn{1}{r|}{{ \textbf{19.1}$^{\dagger}$}} & { \textbf{25.6}$^{\dagger \ddagger}$}           & { \textbf{25.92}$^{\dagger \ddagger}$}            \\ \hline
\multicolumn{1}{|l|}{{ Supervised - CopyRNN}} & { 29.6}                    & \multicolumn{1}{r|}{{ 29.8}}          & { 22.7}                    & \multicolumn{1}{r|}{{ 23.5}}          & { 37.2}                    & \multicolumn{1}{r|}{{ 34.1}}         & { 30.1}                    & \multicolumn{1}{r|}{{ 24.5}}          & { 30.6}                    & \multicolumn{1}{r|}{{ 25.6}}          & { 30.04}                   & { 27.5}                      \\ \hline
\multicolumn{13}{|c|}{{ \textbf{Absent keyphrase generation}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
\multicolumn{1}{|l|}{{ }}                     & \multicolumn{2}{c|}{{ SemEval}}                                                        & \multicolumn{2}{c|}{{ Inspec}}                                                         & \multicolumn{2}{c|}{{ NUS}}                                                           & \multicolumn{2}{c|}{{ Krapivin}}                                                       & \multicolumn{2}{c|}{{ KP20K}}                                                          & \multicolumn{2}{c|}{{ Avg}}                                                   \\ \cline{2-13} 
\multicolumn{1}{|l|}{\multirow{-2}{*}{{ }}}   & \multicolumn{1}{c}{{ R@5}} & \multicolumn{1}{c|}{{ R@10}}          & \multicolumn{1}{c}{{ R@5}} & \multicolumn{1}{c|}{{ R@10}}          & \multicolumn{1}{c}{{ R@5}} & \multicolumn{1}{c|}{{ R@10}}         & \multicolumn{1}{c}{{ R@5}} & \multicolumn{1}{c|}{{ R@10}}          & \multicolumn{1}{c}{{ R@5}} & \multicolumn{1}{c|}{{ R@10}}          & \multicolumn{1}{c}{{ R@5}} & \multicolumn{1}{c|}{{ R@10}} \\ \hline
\multicolumn{1}{|l|}{{ AutoKeyGen}}           & { 0.7}                     & \multicolumn{1}{r|}{{ 1.2}}           & { 1.7}                     & \multicolumn{1}{r|}{{ 2.8}}           & { 2.3}                     & \multicolumn{1}{r|}{{ 3.2}}          & { 2.4}                     & \multicolumn{1}{r|}{{ 3.8}}           & { {\ul 2.2}}               & \multicolumn{1}{r|}{{ {\ul 3.6}}}     & { 1.86}                    & { 2.92}                      \\
\multicolumn{1}{|l|}{{ UOKG}}                 & { {\ul 1.4}}               & \multicolumn{1}{r|}{{ {\ul 2.2}}}     & { {\ul 2}}                 & \multicolumn{1}{r|}{{ {\ul 2.9}}}     & { {\ul 2.7}}               & \multicolumn{1}{r|}{{ {\ul 3.9}}}    & { \textbf{4.5}}            & \multicolumn{1}{r|}{{ \textbf{7.1}}}  & { 1.9}                     & \multicolumn{1}{r|}{{ 2.9}}           & { {\ul 2.5}}               & { {\ul 3.8}}                 \\
\multicolumn{1}{|l|}{{ \textbf{ERU-KG}}}      & { \textbf{1.9}$^{\ddagger}$}            & \multicolumn{1}{r|}{{ \textbf{2.5}$^{\ddagger}$}}  & { \textbf{4.9}$^{\dagger \ddagger}$}            & \multicolumn{1}{r|}{{ \textbf{5.9}$^{\dagger \ddagger}$}}  & { \textbf{3.9}$^{\ddagger}$}            & \multicolumn{1}{r|}{{ \textbf{5.9}$^{\dagger \ddagger}$}} & { {\ul 4.4}$^{\ddagger}$ }              & \multicolumn{1}{r|}{{ {\ul 5.9}$^{\dagger \ddagger}$}}     & { \textbf{5.4}$^{\dagger \ddagger}$}            & \multicolumn{1}{r|}{{ \textbf{7.4}$^{\dagger \ddagger}$}}  & { \textbf{4.1}$^{\dagger \ddagger}$}            & { \textbf{5.52}$^{\dagger \ddagger}$}             \\ \hline
\multicolumn{1}{|l|}{{ Supervised - CopyRNN}} & { 2.1}                     & \multicolumn{1}{r|}{{ 2.7}}           & { 3.7}                     & \multicolumn{1}{r|}{{ 5.2}}           & { 5.9}                     & \multicolumn{1}{r|}{{ 7.8}}          & { 7.9}                     & \multicolumn{1}{r|}{{ 10.8}}          & { 7.1}                     & \multicolumn{1}{r|}{{ 9.4}}           & { 5.34}                    & { 7.18}                      \\ \hline
\end{tabular}
}
\caption{Keyphrase generation performances on five benchmark datasets. The best results are bolded, while the second-best are highlighted. Experiments for AutoKeyGen, UOKG, CopyRNN, and our method are conducted five times, with the average results reported. Both F1 and Recall are presented as percentages. $^\dagger$ and $^\ddagger$ indicate significance
over UOKG and AutoKeyGen with $p<0.01$, respectively.}
\label{table:keyphrase_generation_performance}
\end{table*}

==> latex/tables/ablation_studies_absent_kps.tex <==
\begin{table*}[h]
\centering
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{|c|l|cccccc|}
\hline
Type &
  Model &
  SCIDOCS &
  SciFact &
  TREC-COVID &
  NFCorpus &
  DORIS-MAE &
  ACM-CR \\ \hline
 &
  AutoKeyGen &
  \cellcolor[HTML]{EFAEA9}-2.7 &
  \cellcolor[HTML]{E3F4EC}0.1 &
  \cellcolor[HTML]{EFACA6}-9.3 &
  \cellcolor[HTML]{7BCAA3}10 &
  \cellcolor[HTML]{F2BDB9}-1 &
  \cellcolor[HTML]{E99089}-1.6 \\
 &
  UOKG &
  \cellcolor[HTML]{FBEDEB}-0.6 &
  \cellcolor[HTML]{FFFFFF}0 &
  \cellcolor[HTML]{F6D4D1}-4.8 &
  \cellcolor[HTML]{8BD0AE}8.8 &
  \cellcolor[HTML]{E67C73}-2 &
  \cellcolor[HTML]{E67C73}-1.9 \\
 &
  TPG &
  \cellcolor[HTML]{F2BDB9}-2.2 &
  \cellcolor[HTML]{F2BDB9}-0.3 &
  \cellcolor[HTML]{F8DBD8}-4 &
  \cellcolor[HTML]{AFDFC7}6.1 &
  \cellcolor[HTML]{FDF8F8}-0.1 &
  \cellcolor[HTML]{F0B3AD}-1.1 \\
 &
  CopyRNN &
  \cellcolor[HTML]{E67C73}-4.4 &
  \cellcolor[HTML]{E67C73}-0.6 &
  \cellcolor[HTML]{E67C73}-14.7 &
  \cellcolor[HTML]{6EC59A}11 &
  \cellcolor[HTML]{CDEBDC}0.6 &
  \cellcolor[HTML]{EDA59F}-1.3 \\
\multirow{-5}{*}{Query} &
  ERU-KG-base &
  \cellcolor[HTML]{B7E2CD}1.9 &
  \cellcolor[HTML]{E3F4EC}0.1 &
  \cellcolor[HTML]{FFFFFF}0 &
  \cellcolor[HTML]{57BB8A}12.7 &
  \cellcolor[HTML]{E6F5EE}0.3 &
  \cellcolor[HTML]{F7D5D2}-0.6 \\ \hline
 &
  AutoKeyGen &
  \cellcolor[HTML]{FCFEFD}0.1 &
  \cellcolor[HTML]{FFFFFF}0 &
  \cellcolor[HTML]{FEFDFD}-0.2 &
  \cellcolor[HTML]{FFFFFF}0 &
  \cellcolor[HTML]{F2BDB9}-1 &
  \cellcolor[HTML]{FBEAE8}-0.3 \\
 &
  UOKG &
  \cellcolor[HTML]{E1F3EA}0.8 &
  \cellcolor[HTML]{E3F4EC}0.1 &
  \cellcolor[HTML]{FEFFFF}0.1 &
  \cellcolor[HTML]{FCFEFD}0.3 &
  \cellcolor[HTML]{FCF1F1}-0.2 &
  \cellcolor[HTML]{F7FCF9}0.1 \\
 &
  CopyRNN &
  \cellcolor[HTML]{FCFEFD}0.1 &
  \cellcolor[HTML]{F2BDB9}-0.3 &
  \cellcolor[HTML]{FFFFFF}0 &
  \cellcolor[HTML]{FEFFFF}0.1 &
  \cellcolor[HTML]{FAE4E3}-0.4 &
  \cellcolor[HTML]{F4C7C4}-0.8 \\
\multirow{-4}{*}{Doc} &
  ERU-KG-base &
  \cellcolor[HTML]{85CEAA}3.2 &
  \cellcolor[HTML]{E3F4EC}0.1 &
  \cellcolor[HTML]{FBEDEB}-2 &
  \cellcolor[HTML]{EDF8F3}1.4 &
  \cellcolor[HTML]{E88981}-1.8 &
  \cellcolor[HTML]{C2E6D4}0.7 \\ \hline
\end{tabular}
}
\caption{Impact of including absent keyphrases to expansions on \textit{text retrieval} performance. Colors represent performance changes: \hlc{ablationgreen}{green} indicates an increase, and \hlc{ablationred}{red} indicates a decrease in \textbf{R@1000} compared to excluding absent keyphrases. \lamdo{Add number of absent terms added}}
\label{table:ablation_studies_absent_kps}
\end{table*}

==> latex/tables/classification_based_evaluation.tex <==
\begin{table}[]
\centering

\resizebox{0.75\columnwidth}{!}{\begin{tabular}{|l|cc|}
\hline
               & Arxiv CSMC & Field of study \\ \hline
no expansion   & 49.3       & 42.5           \\ \hline
+ AutoKeyGen   & 47.8       & 41.6           \\
+ UOKG         & 48.4       & 42             \\
+ CopyRNN      & 48.7       & 42.1           \\
+ ERU-KG-small & 48.2       & 44             \\
+ ERU-KG-base  & 48.8       & 45.1           \\ \hline
\end{tabular}}
\caption{}
\label{table:classification_based_evaluation}
\end{table}
